Persistent Backdoor Attacks in Continual Learning

Backdoor attacks pose a significant threat to neural networks, enabling adversaries to manipulate model outputs on specific inputs, often with devastating consequences, especially in critical applications. While backdoor attacks have been studied in various contexts, little attention has been given to their practicality and persistence in continual learning, particularly in understanding how the continual updates to model parameters, as new data distributions are learned and integrated, impact the effectiveness of these attacks over time. To address this gap, we introduce two persistent backdoor attacks-Blind Task Backdoor and Latent Task Backdoor-each leveraging minimal adversarial influence. Our blind task backdoor subtly alters the loss computation without direct control over the training process, while the latent task backdoor influences only a single task's training, with all other tasks trained benignly. We evaluate these attacks under various configurations, demonstrating their efficacy with static, dynamic, physical, and semantic triggers. Our results show that both attacks consistently achieve high success rates across different continual learning algorithms, while effectively evading state-of-the-art defenses, such as SentiNet and I-BAU.

==> 2-Motivation.tex <==
\section{Motivation}
\label{sec: motivation}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures2/BadNet_Attack.png} 
%   \caption{Attack Success Rate for Active Attack}
%   \label{fig:BadNet_Attack}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures2/Active_Attack_ACC.png} 
%   \caption{Classification Rate at clear images for Active Attack}
%   \label{fig:BadNet_Attack}
% \end{figure}


\begin{figure}
  \includegraphics[width=0.9\columnwidth]{PPT-PDF/Motivation-pptx.pdf} 
  \caption{Presenting backdoor attacks such as BadNet and dynamic backdoor in continual learning tasks, the attention heatmap graphs reveal two algorithm failures. For both algorithms, the original images are labeled as dogs. Initially, the attention map for Task sequence 1 shows success for both BadNet and dynamic backdoor algorithms. However, as the continual learning process progresses, the BadNet backdoor fails at Task sequences 3 and 5, and the dynamic backdoor fails at Task sequence 5.}
  \label{fig:research_motivation}
\end{figure}

% \begin{figure}
%   \includegraphics[width=0.9\columnwidth]{PPT-PDF/introduction.png} 
%   \caption{Present backdoor attacks, \,  e.g., BadNet, dynamic backdoor, etc., demonstrate failures in attacking various continual learning algorithms. Two graphs illustrate the failures of LwF, DGR, A-GEM, and XdG with two different classification models across two continual learning datasets, highlighting the effectiveness of our proposed attacks.}
%   \label{fig:research_motivation}
% \end{figure}


% \begin{figure}
%   \includegraphics[width=\columnwidth]{PPT-PDF/Motivation2.pdf} 
%   \caption{Illustration of active backdoor attack failures: XdG and DGR are CL algorithms that suffer from active backdoor attacks. ASR is the attack success rate, and ACC is the accuracy rate at a clear dataset. Timeline stands for CL training stream. Each plot line shows ASR variations after succeeding tasks.}
%   \label{fig:Motivation2}
% \end{figure}

In the past two years, some papers show CL is vulnerable to suffering from data-poisoning attacks \cite{poision-ewc-si}, \cite{dgr-poisoning}, \cite{brainWash}. Poisoning-based backdoor attacks in the context of CL have yet to be researched extensively, leaving potential security risks. Yiqi, etc. \cite{backdoor-CL-study} had empirically evaluated the performance of poisoning-based and non-target backdoor attacks against multiple CL algorithms in Task-IL, Domain-IL, and Class-IL. 

This paper comprehensively evaluates \textbf{poisoning-based} and \textbf{target backdoor} attacks in Task-IL and Class-IL. Also, we argue that one of the main possible reasons why some CL algorithms fail is that \textbf{the tiny backdoor trigger}, compared to original image data, is forgotten more possibly and is not focused on learning as the continual learning illustrated by Figure \ref{fig:research_motivation}. Inspired by this, we first design a novel attack model against poisoning-based and target backdoor attacks. The top row of Figure \ref{fig:research_motivation} depicts the standard Task-IL procedure. During Task 1, which involves processing handwriting images labeled 0 and 1, we obtain the model $F_{\theta}^1$. For Task 2, which processes handwriting images labeled 2 and 3, the model $F_{\theta}^2$ is obtained not from scratch but by building upon $F_{\theta}^1$. This is visually indicated by the neural colors, with the green neurons representing those inherited from Task 1. Subsequent tasks follow this pattern, significantly conserving the time and computational resources required for learning new data. In practice, the deep learning model and training data outsourcing to remote machine learning cloud servers, such as Amazon, is employed when local computer capabilities are insufficient for model training. This scenario presents a potential vulnerability to attackers. They compromise the model $F_{\theta}^1$, embedding a crafted trigger in certain images, which results in their misclassification under a designated target label. As depicted in Figure \ref{fig:research_motivation}, the model $F_{\theta}^1$ is manipulated into $F_{\theta}^{'1}$. This is evidenced by the color change of the neural at the bottom from green to grey, indicating the model's $F_{\theta}^{'1}$ acquisition of the trigger. During the CL process, the attacking efficiency of the grey neural diminishes, reaching its lowest point in the final task. 

Some CL algorithms have demonstrated diminishing attack efficiency at cross-task learning, resulting in the failure of CL in the context of these attacks despite initial success in poisoning-based backdoor attacks. Figure \ref{fig:Motivation2} illustrates the ineffectiveness of attacks against XdG and DGR algorithms. The blue line in legend represents the starting point of an attack at Task 1, and the green legend indicates the start at Task 2, and so on. Analysis of Figure \ref{fig:Motivation2} reveals that when attacks begin at Task 1, Task 2, or Task 3, the XdG algorithm prioritizes maintaining a high Attack Success Rate (ASR) at the expense of a declining classification Accuracy (ACC). Three of four total attack instances (excluding the final one, which lacks a continuous timeline) are unsuccessful, concluding that backdoor attacks against XdG are mainly ineffective. The gradual decrease in both ASR and ACC further evidences this ineffectiveness. 

Motivated by these, we first comprehensively evaluates poisoning-based and target backdoor attacks in Task-IL and Class-IL and first design a novel attack model against poisoning-based and target backdoor attacks. 


%TODO%

\begin{figure}
  \includegraphics[width=\columnwidth]{Figures/motive1.png} 
  \caption{Schematic graph of research motivation. The left graph is a visualization of the loss function for task 1 of the XDG algorithm (a continual learning algorithm). The starting point of training is $T_0$, and the endpoint is $T_1$ along the black line. The right graph is the visualization of the loss function for task 2, which begins at $T_1$ and ends at $T_2$ along the black line. This direction leads to increasing the loss of task1. However, task1 and task2 would have a minor loss if task2 followed the orange dashed line. And this direction has less change in parameters. The attack would be more successful if we followed this direction with less parameter change. Inspired by this intuition, we constructed a methodology to identify which layer is more stable during continual learning. }
  \label{fig:motive1}
\end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/motivation2.png} 
%   \caption{Parameters variation of three layers for six algorithms. One point shows parameters variation value in $\delta_0$ and $\delta_1$ direction}
%   \label{fig:motivation2}
% \end{figure}

Figure \ref{fig:motive1} shows our motivation of this paper. The left graph is a visualization of the loss function for task 1 of the XDG algorithm (a continual learning algorithm). The starting point of training is T0, and the endpoint is T1 along the black line. The right graph is the visualization of the loss function for task 2, which begins at T1 and ends at T2 along the black line. This direction leads to increasing the loss of task1. However,
task1 and task2 would have a minor loss if task2 followed the orange dashed line. And this direction has less change in parameters. The attack would be more successful if we followed this direction with less parameter change. Inspired by this intuition, we constructed a methodology to identify which layer is more stable during continual learning.


==> 7-RelatedWork.tex <==
\section{Related Work}

%\subsection{Backdoor Attacks}
In recent years, \cite{goldblum2022dataset,Nguyen2020InputAwareDB,nguyen-2020} explore the dynamic trigger to increase the stealthiness of backdoor attacks, demonstrating that these methods could evade conventional detection mechanisms by varying trigger patterns over time. \cite{Turner2018CleanLabelBA, Zhao2020CleanLabelBA, zhao2022clean, narcissus-2023} investigate clean-label attacks, which do not require label change, making them harder to detect and prevent. Khaddaj et al. \cite{khaddaj2023rethinking} propose a novel approach to backdoor attacks in deep learning models by exploiting naturally occurring features in the dataset, which act as inadvertent triggers. 

As for the continual learning scenarios, \cite{Umer2021AdversarialTF, Li2022TargetedDP, Umer2020TargetedFA} explore backdoor attacks in continual learning by injecting poisoning samples. In contrast, our research employs a trigger-based backdoor, which is distinct from poisoning data. Moreover, our research goals differ from theirs, as their primary objective is to enhance the forgetting rate of knowledge learned in previous tasks~\cite{Bagdasaryan2018HowTB, Sun2019CanYR, Wang2020AttackOT} investigate backdoor attacks in federated learning, with \cite{Xie2020DBADB} designing a distributed backdoor attack in the same context. Recently,~\cite{fang2023vulnerability} introduced a new federated backdoor attack framework that modifies local model weights to inject the backdoor trigger. However, our work is focused on the continual learning scenario, distinguishing it from the aforementioned studies.

%\subsection{Backdoor Attacks in Continual Learning}
% Backdoor attacks in continual learning scenarios are a growing area of research. CL models are particularly vulnerable to backdoor attacks because they need to learn new tasks incrementally. Liu et al. highlight the susceptibility of regularization-based CL algorithms, such as EWC and SI, to data poisoning attacks, emphasizing the need for robust defense mechanisms \cite{liu2022data}. Umer et al. (2022) propose a method to introduce imperceptible backdoor triggers that exploit the continual learning process to form false memories, making detection and mitigation more challenging \cite{umer2022false}. 


% Our work builds on these foundations by exploring parameter variations in neurons across different tasks and layers in six continual learning algorithms. We propose strategies to leverage neurons with minimal variations for embedding trigger information. Our \waa only needs to adjust one task, enhancing the stealthiness of backdoor attacks in continual learning scenarios.


==> comments.tex <==
% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/cosines.png} 
%   \caption{Similarity of three layers for six algorithms. $t_{12}$ at leftest graphs indicates task$1$ and task$2$ for layer$1$}
%   \label{fig:cosines}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/kdes.png} 
%   \caption{Kernel density graph for six algorithms. $t_{12}$ at leftest graphs indicates task$1$ and task$2$ for layer$1$}
%   \label{fig:kdes}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/XDG_weight_variation.png} 
%   \caption{Parameters variation of three layers of XDG. The variation value of layer3 is smallest but the values of all three layers are bigger than SI.}
%   \label{fig:XDG_weight_variation}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/SI_weight_variation2.png} 
%   \caption{Changes in the position of parameters of neural network from task1 to task5 for SI continual learning after principle component analysis. dist:2.7 shows the cumulative variation in parameters is 2.7.}
%   \label{fig:SI_weight_variation2}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/XDG_weight_variation2.png} 
%   \caption{Changes in the position of parameters of neural network from task1 to task5 for XDG continual learning after principle component analysis.}
%   \label{fig:XDG_weight_variation2}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/SI_KDE3.png} 
%   \caption{Parameters kernel density of neural network from task1 to task5 for SI continual learning after principle component analysis and threshold 0.8 filter. Layer1 to layer3 from top row to bottom.}
%   \label{fig:SI_KDE3}
% \end{figure}


% \begin{figure}
%   \includegraphics[width=\columnwidth]{Figures/XDG_KDE3.png} 
%   \caption{Parameters kernel density of neural network from task1 to task5 for XDG continual learning after principle component analysis and threshold 0.8 filter. Layer1 to layer3 from top row to bottom.}
%   \label{fig:XDG_KDE3}
% \end{figure}
